Optimal Dyck Reachability for Data-Dependence and Alias Analysis

A fundamental algorithmic problem at the heart of static analysis is Dyck reachability. The input is a graph where the edges are labeled with different types of opening and closing parentheses, and the reachability information is computed via paths whose parentheses are properly matched. We present new results for Dyck reachability problems with applications to alias analysis and data-dependence analysis. Our main contributions, that include improved upper bounds as well as lower bounds that establish optimality guarantees, are as follows. First, we consider Dyck reachability on bidirected graphs, which is the standard way of performing field-sensitive points-to analysis. Given a bidirected graph with $n$ nodes and $m$ edges, we present: (i)~an algorithm with worst-case running time $O(m + n \cdot \alpha(n))$, where $\alpha(n)$ is the inverse Ackermann function, improving the previously known $O(n^2)$ time bound; (ii)~a matching lower bound that shows that our algorithm is optimal wrt to worst-case complexity; and (iii)~an optimal average-case upper bound of $O(m)$ time, improving the previously known $O(m \cdot \log n)$ bound. Second, we consider the problem of context-sensitive data-dependence analysis, where the task is to obtain analysis summaries of library code in the presence of callbacks. Our algorithm preprocesses libraries in almost linear time, after which the contribution of the library in the complexity of the client analysis is only linear, and only wrt the number of call sites. Third, we prove that combinatorial algorithms for Dyck reachability on general graphs with truly sub-cubic bounds cannot be obtained without obtaining sub-cubic combinatorial algorithms for Boolean Matrix Multiplication, which is a long-standing open problem. We also show that the same hardness holds for graphs of constant treewidth.

==> lower_bound_old.tex <==
\smallskip\noindent{\bf Conditional reachability.}
Given a $\Alphabet$-labeled graph $G=(V,E)$ and four nodes $w,x,y,z\in V$,
we say that $z$ is \emph{Dyck-reachable from} $w$ \emph{via} $x,y$, denoted $\CondReach(w,x,y,z)$,
if $z$ is Dyck-reachable from $w$, and every $w,z$-witness path $P$ contains a $x,y$-witness subpath $P':x\Path y$.
Intuitively, every witness path from $w$ to $z$ contains a witness subpath from $x$ to $y$.

\smallskip\noindent{\bf Monotonic Bidirected Reachability algorithms.}
We define a class $\mathcal{A}$ of \emph{monotonic Bidirected Reachability algorithms}  that solve the Bidirected Reachability problem.
An algorithm $A$ with state space $S_{A}$ belongs to $\mathcal{A}$ if there exists a map $f:S_{A}\to \{\True, \False\}^{V\times V}$
such that for every computation of $A$ on some input $G=(V,E)$ that produces the sequence of states $S_1,\dots S_r$, the following conditions hold.
\begin{compactenum}
\item If there exists some $i$ and a pair of nodes $u,v$ such that $f(S_i)(u,v)=\True$, then for all $j\geq i$ we have $f(S_i)(u,v)=\True$.
\item For any four nodes $w,x,y,z$ such that $\CondReach(w,x,y,z)$, there exists some $i$ such that $f(S_i)(x,y)=\True$ and $f(S_i)(w,z)=\False$.
\item For every pair of nodes $u,v$, we have $f(S_r)(u,v)=\True$ iff $u$ and $v$ belong to the same DSCC of $G$.
\end{compactenum}

Intuitively, an algorithm is called monotonic if, in order to discover in some state $S_i$ that a node $z$ is Dyck-reachable from another node $w$ via a path $w\Path x\Path y\Path z$,
the algorithm must have discovered in some previous state that $y$ is Dyck-reachable from $x$.
Hence the monotonicity concerns the length of the paths that are witnesses of reachability information.
All existing algorithms for Bidirected Reachability are monotonic~\cite{Yuan09,Zhang13},
and the map $f$ is typically maintained explicitly by the algorithm as a data structure.



\smallskip\noindent{\bf  3-access sequences.}
A sequence of union-find operations $\sigma$ over a set $X$ is called \emph{3-access} if the following conditions hold.
\begin{compactenum}
\item\label{item:three_operations} Every element of $A$ appears in at most three operations of $\sigma$.
\item\label{item:nontrivial_union} For every index $i$, if $\sigma(i)=\Union(u,v)$ then the elements $u$, $v$ belong to different sets
after the prefix of $\sigma$ up to position $i-1$ has been executed.
Hence the $\Union$ operation in position $i$ is a non-trivial one.
\end{compactenum}
 

\begin{lemma}\label{lem:three_access_hard}
Any algorithm for the Union-Find problem over 3-access  sequences requires $\Omega(n\cdot \alpha(n))$ time, where $n$ is the length of the input sequence.
\end{lemma}
\begin{proof}
Consider any algorithm $A$ that solves the Union-Find problem over 3-access sequences.
We will describe an algorithm $A'$ that can handle arbitrary sequences using $A$ as an oracle.
Given a sequence $\sigma$ of length $n$, the algorithm $A'$ will be constructing a new, 3-access sequence $\sigma'$.
To handle each new operation of $\sigma$, $A'$ will be querying $A$ on a constant number of operations of $\sigma'$.

We now describe the algorithm $A'$. 
To guarantee \cref{item:nontrivial_union}, the algorithm constructs from $\sigma$ a new sequence $\sigma''$,
where every operation $\Union(x,y)$ is first preceded by two operations $\Find(x)$, $\Find(y)$.
If $\Find(x)\neq \Find(y)$, then $A'$ keeps the operation $\Union(x,y)$ in $\sigma''$, otherwise $A'$ removes $\Union(x,y)$ from $\sigma''$.

We now proceed to describe how to obtain the 3-access sequence $\sigma'$ from $\sigma''$.
The algorithm simply uses a fresh surrogate symbol $x_i\not \in X$ to replace the $i$-th appearance of the symbol $x\in X$ in $\sigma$. We split cases to determine how $A'$ will handle the next operation of $\sigma$, according to the type of the operation.

\begin{compactenum}
\item $\Find(x)$, where $x$ appears for the $i$-th time in $\sigma$.
The algorithm $A'$ introduces a new surrogate symbol $x_i$ and extends $\sigma'$ by the following operations: $\Union(x_{i-1}, x_i)$, $\Find(x_i)$.
Then, it returns the symbol that $A$ returned on $\Find(x_i)$.
\item $\Union(x,y)$, where $x$, $y$ appear for the $i$-th and $j$-th time in $\sigma$, respectively.
The algorithm $A'$ introduces two new surrogate symbols $x_i$, $y_j$, and extends $\sigma'$ by the following operations:
$\Union(x_{i-1}, x_i)$, $\Union(y_{j-1}, y_j)$, $\Union(x_i,y_j)$.
\end{compactenum}

It is easy to see that $\sigma'$ is a 3-access sequence of length at most $3\cdot n$, since every union operation is applied on elements of distinct sets,
and every element $x_i$ is used at most 3 times:
(i)~$\Union(x_{i-1},x_{i})$, (ii)~$\Find(x_i)$ or $\Union(x_i, y_i)$ (iii)~$\Union(x_i, x_{i+1})$.
Finally, it is trivial to establish that $A'$ handles each operation of $\sigma$ correctly.
The total time required for $A'$ to handle $\sigma$ is asymptotically equally to the time required by $A$ to handle $\sigma'$.
Since, by ~\cite{Tarjan79,Banachowski80}, the lower bound for $A'$ is $\Omega(n\cdot \alpha(n))$,
we obtain the same lower bound for the algorithm $A$.

The desired result follows.
\end{proof}







{\bf NOT EXACTLY BIDIRECTED}
\smallskip\noindent{\bf Reduction from the Union-Find problem to Bidirected Reachability.}
Let $X$ be a set of $n$ elements, and $\sigma$ a 3-access union-find sequence over $X$ of length $|\sigma|=n$.
For ease of presentation, we assume wlog that $\sigma$ starts with a $\Union$ operation.
We construct a $\Alphabet_5$-labeled bidirected graph $G^{\sigma}=(V^{\sigma}, E^{\sigma})$ as follows.
\begin{compactenum}
\item $V^{\sigma}=X\cup \{x_i,y_i,z_i: \sigma(i)=\Find(u_i) \} \cup \{x_i, y_i: \sigma(i)=\Union(u_i,v_i)\}$ i.e., $V^{\sigma}$ consists of the elements of $X$, together with three nodes $x_i, y_i, z_i$ associated with each $\Find$ operation of $\sigma$, and two nodes $x_i, y_i$ associated with each $\Union$ operation of $\sigma$.
\item $E^{\sigma}=\bigcup_iE^{\sigma}_i$ where $E^{\sigma}_1=\{(x_1,y_1, \epsilon), (y_1, x_1, \epsilon), (x_1,v_1,\CloseParenthesis_{1}), (y_1,u_1,\CloseParenthesis_{1})\}$,
and the set $E^{\sigma}_i$ depends on the sets $E^{\sigma}_{j<i}$.
For each element $u\in X$ and each positive integer $i\leq n$, we let $\Count(i,u)$ denote the smallest positive integer $\ell$ such that the edge set $\bigcup_{j\leq i}E^{\sigma}_j$ does not contain an edge of $u$ labeled with $\ell$.
Then, for all $2\leq i \leq n$, the set $E^{\sigma}_i$ depends on the type of operations in $\sigma(i-1)$ and $\sigma(i)$, as follows.
\begin{enumerate}
\item $\sigma(i)=\Find(u_i)$, $\sigma(i-1)=\Find(u_{i-1})$, for some $u_i,u_{i-1}\in X$.
Then we have $(x_i,z_i, \CloseParenthesis_{\ell}), (y_i, u_i, \CloseParenthesis_{\ell}), (u_{i-1},y_i, \CloseParenthesis_{j}), (z_{i-1}, x_i, \CloseParenthesis_{j}) \in E^{\sigma}$,
where $j= \Count(i-1,u_{i-1})$ and $\ell=\Count(i-1, u_i)$.

\item $\sigma(i)=\Find(u_i)$, $\sigma(i-1)=\Union(v_{i-1},u_{i-1})$, for some $u_i,v_{i-1},u_{i-1}\in X$.
Then we have $(x_i,z_i, \CloseParenthesis_{\ell}), (y_i, u_i, \CloseParenthesis_{\ell}), (u_{i-1},y_i, \CloseParenthesis_{j}), (v_{i-1}, x_i, \CloseParenthesis_{j}) \in E^{\sigma}$,
where $j=\min_{r}: \Count(i-1,v_{i-1}), \Count(i-1,u_{i-1})\geq r$ and $\ell=\Count(i-1, u_i)$.

\item $\sigma(i)=\Union(u_i,v_i)$, $\sigma(i-1)=\Find(u_{i-1})$, for some $u_i,v_i,u_{i-1}\in X$.
Then we have $(y_i, u_i, \CloseParenthesis_{\ell}), (x_i, v_i, \CloseParenthesis_{\ell}), (u_{i-1}, y_i, \CloseParenthesis_{j}), (z_{i-1}, x_i, \CloseParenthesis_{j})  \in E^{\sigma}$,
where $j= \Count(i-1,u_{i-1})$ and $\ell = \min_{r}: \Count(i-1,v_{i}), \Count(i-1,u_{i})$.

\item $\sigma(i)=\Union(v_i,u_i)$, $\sigma(i-1)=\Union(v_{i-1},u_{i-1})$, for some $u_i,v_i,v_{i-1}, u_{i-1}\in X$.
Then we have $(y_i, u, \CloseParenthesis_{1}), (x_i, v, \CloseParenthesis_{1}), (u_{i-1}, y_i, \CloseParenthesis_{j}), (v_{i-1}, x_i, \CloseParenthesis_{j})  \in E^{\sigma}$,
where $j=\min(\Count(i-1,u_{i-1}), \Count(i-1,v_{i-1}))$ and $\ell = \min_{r}: \Count(i-1,v_{i}), \Count(i-1,u_{i})$.
\end{enumerate}
See \cref{fig:G_sigma} for an illustration. Note that in call cases where $\CloseParenthesis_j$ or $\CloseParenthesis_{\ell}$ is used, we have $j,\ell\leq 5$, and thus $\CloseParenthesis_j \in \Alphabet_5$.
This follows easily from the fact that $\sigma$ is a 3-access sequence, and thus for any positive integer $i$ and any two elements $v,w\in X$ that appear in the operation $\sigma(i)$,  we have $\Count(i,w), \Count(i,v)< 3$. Hence, the smallest value which is at least as large as $\Count(i,w)$ and $\Count(i, v)$ is at most $5$.
\end{compactenum}

\input{figures/G_sigma}

The following remark follows easily from the above construction.

\smallskip
\begin{remark}\label{rem:unique_edge}
For every element $u\in X$ and $\CloseParenthesis_j\in \Alphabet_5$, 
there exists at most one incoming edge and at most one outgoing edge of $u$ labeled with $\CloseParenthesis_j$.
\end{remark}


\smallskip
\begin{lemma}\label{lem:G_simple}
The following assertions hold, for $2\leq i\leq n$.
\begin{compactenum}
\item \label{item:0} $\CondReach(v_1, x_1, y_1, u_1)$.
\item\label{item:1} If $\sigma(i)=\Find(u_i)$ then $\CondReach(z_i, x_i, y_i, u_i)$.
\item\label{item:2} If $\sigma(i)=\Union(v_i, u_i)$ then $\CondReach(v_i, x_i, y_i, u_i)$.
\item\label{item:3} If $\sigma(i-1)=\Find(u_{i-1})$ then $\CondReach(x_i, z_{i-1}, u_{i-1}, y_i)$.
\item\label{item:4} If $\sigma(i-1)=\Union(w_{i-1},u_{i-1})$ then $\CondReach(x_i, v_{i-1}, u_{i-1}, y_i)$.
\end{compactenum}
\end{lemma}
\begin{proof}
We first prove inductively that for all $1\leq i\leq n$, the reachability relations defined by the first and last argument of $\CondReach$ hold.
Recall that $\sigma(1)=\Union(v_1, u_1)$, and since $(v_1,x_1,\epsilon)\in E^{\sigma}$, we have that $u_1$ is Dyck-reachable from $v_1$ via the path $P:v_1\to x_1\to y_1\to u_1$ with label $\Label(P)=\OpenParenthesis_{1}~\epsilon~\CloseParenthesis_{1} \in \Dyck_5$.
Now assume that the claim holds for $i-1$, and we will show it holds for $i$.
We first split cases according to the type of the $i-1$-th operation of $\sigma$.
\begin{compactenum}
\item If $\sigma(i-1)=\Find(u_{i-1})$, then by the induction hypothesis $u_{i-1}$ is Dyck-reachable from $z_{i-1}$.
Since $(x_i, z_{i-1}, \OpenParenthesis_{j}), (u_{i-1}, y_i, \CloseParenthesis_{j})\in E^{\sigma}$, we obtain that $y_i$ is Dyck-reachable from $x_i$,
which proves the reachability statement of \cref{item:3}.
\item If $\sigma(i-1)=\Union(v_{i-1}, u_{i-1})$, then by the induction hypothesis $u_{i-1}$ is Dyck-reachable from $v_{i-1}$.
Since $(x_i, v_{i-1}, \OpenParenthesis_{j}), (u_{i-1}, y_i, \CloseParenthesis_{j})\in E^{\sigma}$, we obtain that $y_i$ is Dyck-reachable from $x_i$,
which proves the reachability statement of \cref{item:4}.
\end{compactenum}
Hence for either type of operation of $\sigma(i-1)$, we have that $y_i$ is reachable from $x_i$.
We now split cases according to the type of the $i$-th operation of $\sigma$.
\begin{compactenum}
\item If $\sigma(i)=\Find(u_i)$, since $(z_i, x_i, \OpenParenthesis_{1}), (y_i, u_i, \CloseParenthesis_{1})\in E^{\sigma}$, we obtain that $u_i$ is Dyck-reachable from $z_i$,
which proves the reachability statement of \cref{item:1}.
\item If $\sigma(i)=\Union(v_i, u_i)$, since $(v_i, x_i, \OpenParenthesis_{1}), (y_i, u_i, \CloseParenthesis_{1})\in E^{\sigma}$, we obtain that $u_i$ is Dyck-reachable from $v_i$,
which proves the reachability statement of \cref{item:2}.
\end{compactenum}
The above concludes the proof that for all $1\leq i \leq n$, for every reachability statement $\CondReach(w,x,y,z)$ made in \cref{item:0}-\cref{item:4}, $z$ is indeed Dyck-reachable from $w$.

We now turn our attention to proving that for every statement $\CondReach(w,x,y,z)$ made in \cref{item:0} - \cref{item:4},
$z$ is indeed Dyck-reachable from $w$ via $x,y$.
The statement is trivially true for \cref{item:3}, since if $\sigma(i-1)=\Find(u_{i-1})$, the edge $(x_i, z_{i-1})$ is the only outgoing edge of $x_i$, and the edge $(u_{i-1}, y_i)$ is the only incoming edge of $y_i$. As $y_i$ is reachable from $x_i$, we have that $\CondReach(x_i, z_{i-1}, u_{i-1}, y_i)$.
Similarly, the statement is trivially true for \cref{item:4}, since if $\sigma(i-1)=\Union(w_{i-1},u_{i-1})$, the edge $(x_i, v_{i-1})$ is the only outgoing edge of $x_i$, and the edge $(u_{i-1}, y_i)$ is the only incoming edge of $y_i$. As $y_i$ is reachable from $x_i$, we have that $\CondReach(x_i, v_{i-1}, u_{i-1}, y_i)$.

It remains to prove the statement for \cref{item:0}-\cref{item:2}.
We split cases based on the type of operation $\sigma(i)$ (thus handling \cref{item:0} and \cref{item:2} simultaneously).

\begin{compactenum}
\item If $\sigma(i)=\Find(u_i)$ then clearly $\CondReach(z_i, x_i, y_i, u_i)$ holds, as $z_i$ has a single outgoing edge $e$, which is to $x_i$
and by \cref{rem:unique_edge} $u_i$ has a single edge incoming edge labeled with $\Label(e)$, which is from $y_i$.

\item If $\sigma(i)=\Union(v_i, u_i)$, it follows easily from \cref{rem:unique_edge} that if $\CondReach(v_i, x_i, y_i, u_i)$ does not hold,
then there exists some $j\neq i$ and a path $P:v_i, x_j, y_j, u_j$.
This implies that there are two union operations $\sigma(i)=\Union(v_i, u_i)$, $\sigma(j)=(v_j, u_j)$ such that $v_i=v_j$ and $x_i=x_j$,
which violates \cref{item:nontrivial_union} of the 3-access sequences which requires that every $\Union$ operation is non-trivial.
\end{compactenum}

We have concluded that every statement $\CondReach(w,x,y,z)$ made in \cref{item:0} - \cref{item:4} is correct,
which concludes the proof of the lemma.
\end{proof}


\smallskip
\begin{theorem}\label{them:bidirected_lower}
Let $G=(V,E)$ be a $\Alphabet$-labeled bidirected graph of $n$ nodes and $m=\Omega(n)$ edges.
Any monotonic Bidirected Reachability algorithm for $G$ requires $\Omega(m+n\cdot \alpha(n))$ time.
\end{theorem}


\smallskip
\begin{corollary}\label{cor:bidirected_optimal}
The algorithm $\BidirectedAlgo$ is optimal in the class of monotonic Bidirected Reachability algorithms.
\end{corollary}







